Gapped Clique Homology on weighted graphs is $\text{QMA}_1$-hard and contained in $\text{QMA}$

We study the complexity of a classic problem in computational topology, the homology problem: given a description of some space $X$ and an integer $k$, decide if $X$ contains a $k$-dimensional hole. The setting and statement of the homology problem are completely classical, yet we find that the complexity is characterized by quantum complexity classes. Our result can be seen as an aspect of a connection between homology and supersymmetric quantum mechanics. We consider clique complexes, motivated by the practical application of topological data analysis (TDA). The clique complex of a graph is the simplicial complex formed by declaring every $k+1$-clique in the graph to be a $k$-simplex. Our main result is that deciding whether the clique complex of a weighted graph has a hole or not, given a suitable promise on the gap, is $\text{QMA}_1$-hard and contained in $\text{QMA}$. Our main innovation is a technique to lower bound the eigenvalues of the combinatorial Laplacian operator. For this, we invoke a tool from algebraic topology known as \emph{spectral sequences}. In particular, we exploit a connection between spectral sequences and Hodge theory. Spectral sequences will play a role analogous to perturbation theory for combinatorial Laplacians. In addition, we develop the simplicial surgery technique used in prior work. Our result provides some suggestion that the quantum TDA algorithm \emph{cannot} be dequantized. More broadly, we hope that our results will open up new possibilities for quantum advantage in topological data analysis.

==> Acknowledgement.tex <==
\section*{Acknowledgement}
The authors would like to thank Marcos Crichigno for suggesting the use of spectral sequences and Forman's theory, and for insightful discussion and collaboration at some stages of the project.
RK is supported by a grant from the Simons Foundation (Simons Investigator Award No. 828076) and the IQIM, an NSF Physics Frontiers Center (NSF Grant PHY-1125565).
TK is supported by the DOE QuantISED grant DE-SC0020360, SLAC (Q-NEXT), QFARM and the Spanish Ministry of Science and Innovation through the “Severo Ochoa Program for Centres of Excellence in R\&D” (CEX2019-00904-S) and PID2020-113523GB-I0.


==> Spectral_sequences_1.0.tex <==
\section{Spectral sequences}\label{spec_seq_sec}

Spectral sequences are a tool from algebraic topology which (among other things) analyze the homology of \emph{filtered} chain complexes. It turns out that weighting a subset of vertices by $\lambda \ll 1$, as we do in our construction, naturally gives rise to a certain filtration. In this setting, Robin Forman 1992 \cite{forman1994hodge} showed a beautiful relationship between the spectral sequence and the perturbative eigenspaces of the Hodge theoretic Laplacian. It is this relationship which we exploit in this section to prove Lemma \ref{spec_seq_lemma}. In introducing these concepts, we will follow \cite{forman1994hodge} closely.

\subsection{Spectral sequence of a filtration}

Spectral sequences will work best for us in the \emph{cohomology} picture. First we define a \emph{filtration}.

\begin{definition}
Suppose we have a cohomological chain complex
\begin{equation*}
\begin{tikzcd}
\mathcal{C}^{-1} \arrow[r,"d^{-1}"] & \mathcal{C}^0 \arrow[r,"d^0"] & \mathcal{C}^1 \arrow[r,"d^1"] & \mathcal{C}^2 \arrow[r,"d^2"] & \dots
\end{tikzcd}
\end{equation*}
A \emph{filtration} on this chain complex is a nested sequence of subspaces
\begin{equation*}
\mathcal{C}^k = \mathcal{U}_0^k \supseteq \mathcal{U}_1^k \supseteq \mathcal{U}_2^k \supseteq \dots
\end{equation*}
for each $n$ such that
\begin{equation*}
d^k(\mathcal{U}_j^k) \subseteq \mathcal{U}_j^{k+1}
\end{equation*}
By convention, $\mathcal{C}^k = \mathcal{U}_{-1}^k = \mathcal{U}_{-2}^k = \dots$.
\end{definition}

We can now define the spectral sequence of such a filtration.

\begin{definition}
Let $\mathcal{C}^k = \mathcal{U}_0^k \supseteq \mathcal{U}_1^k \supseteq \mathcal{U}_2^k \supseteq \dots$ be a filtered chain complex with coboundary $d$. Define
\begin{align*}
Z_{j,l}^k &= \mathcal{U}_l^k \cap (d^k)^{-1}(\mathcal{U}_{l+j}^{k+1}) \\
B_{j,l}^k &= \mathcal{U}_l^k \cap d^{k-1}(\mathcal{U}_{l-j}^{k-1}) \\
e_{j,l}^k &= Z_{j,l}^k / (B_{j-1,l}^k + Z_{j-1,l+1}^k) \\
e_j^k &= \sum_l e_{j,l}^k
\end{align*}
The sequence of spaces $\{e_j^k\}$ is the \emph{spectral sequence}.
\end{definition}

Note that morally we have
\begin{align*}
Z_{\infty,l}^k &= \mathcal{U}_l^k \cap \ker{d^k} \\
B_{\infty,l}^k &= \mathcal{U}_l^k \cap \im{d^{k-1}}
\end{align*}
which gives
\begin{equation*}
e_{\infty}^k = H^k(\mathcal{C}).
\end{equation*}
We also have the series of inclusions
\begin{equation*}
B_{0,l}^k \subseteq B_{1,l}^k \subseteq \dots \subseteq B_{\infty,l}^k \subseteq Z_{\infty,l}^k \subseteq \dots \subseteq Z_{1,l}^k \subseteq Z_{0,l}^k.
\end{equation*}

It can be checked that indeed
\begin{align*}
Z_{j-1,l+1}^k &\subseteq Z_{j,l}^k \\
B_{j-1,l}^k &\subseteq Z_{j,l}^k
\end{align*}
so that the definition of $e_{j,l}^k$ makes sense.


\subsection{Relationship to Hodge theory}

From our construction we have a clique complex $\mathcal{G}$ where a subset of the vertices are weighted by $\lambda \ll 1$, and the rest by $1$. In this context, there is a natural filtration on the chain complex $\mathcal{C}$. Let
\begin{equation*}
\mathcal{U}_j^k = \text{span}\{\sigma \in \mathcal{G}^k : w(\sigma) \in \{\lambda^j,\lambda^{j+1},\dots\}\}
\end{equation*}
Equivalently, this is the span of the $k$-simplices which involve at least $j$ weight-$\lambda$ vertices. These spaces are clearly nested
\begin{equation*}
\mathcal{C}^k = \mathcal{U}_0^k \supseteq \mathcal{U}_1^k \supseteq \mathcal{U}_2^k \supseteq \dots
\end{equation*}
and it can also be checked that
\begin{equation*}
d^k(\mathcal{U}_j^k) \subseteq \mathcal{U}_j^{k+1}
\end{equation*}
Thus we have a filtration.

We are interested in the low energy eigenstates of the Laplacian $\Delta^k$ of $\mathcal{G}$. In particular, we would like to examine the eigenvalues which are zero to first order in $\lambda$, and then second order, and so on. This is reminiscent of perturbation theory from quantum mechanics. Recall that
\begin{equation*}
\langle\psi|\Delta^k|\psi\rangle = ||\partial^k|\psi\rangle||^2 + ||d^k|\psi\rangle||^2
\end{equation*}
Motivated by this, define the isomorphism
\begin{align*}
\rho^k_\lambda : \mathcal{C}^k &\rightarrow \mathcal{C}^k \\
\mathcal{U}_j^k \cap (\mathcal{U}_{j+1}^k)^\perp &\rightarrow \lambda^j \ \mathcal{U}_j^k \cap (\mathcal{U}_{j+1}^k)^\perp
\end{align*}
and the maps
\begin{align*}
\partial^k_\lambda &= \rho^k_\lambda \circ \partial^k \circ (\rho^k_\lambda)^{-1} \\
d^k_\lambda &= \rho^k_\lambda \circ d^k \circ (\rho^k_\lambda)^{-1}
\end{align*}
($\rho_\lambda^k$ is the inverse of the map $\tau_\lambda^k$ which appeared in the proof of Theorem \ref{main_thm}.) Now define the spaces
\begin{align*}
E_j^k = \{|\psi\rangle \in \mathcal{C}^k \ &: \ \exists |\psi_\lambda\rangle = |\psi\rangle + \lambda|\psi_1\rangle + \lambda^2|\psi_2\rangle + \dots + \lambda^j|\psi_j\rangle \\
&\text{s.t.} \ \partial^k_\lambda|\psi_\lambda\rangle \in \lambda^j \mathcal{C}^{k-1}[\lambda] , \ d^k_\lambda|\psi_\lambda\rangle \in \lambda^j \mathcal{C}^{k+1}[\lambda]\}
\end{align*}
and
\begin{equation*}
E_{j,l}^k = E_j^k \cap \mathcal{U}_l^k \cap (\mathcal{U}_{l+1}^k)^\perp
\end{equation*}
so that
\begin{equation*}
E_j^k = \sum_l E_{j,l}^k
\end{equation*}
where $\mathcal{C}^k[\lambda]$ is the space of polynomials in $\lambda$ with coefficients in $\mathcal{C}^k$. $E_j^k$ is the space of vectors which have perturbations in $\lambda$ which give eigenvalues of size $\mathcal{O}(\lambda^j)$. Morally, taking $j\rightarrow\infty$ should give $E_\infty^k = H^k(\mathcal{C})$.

Theorem 7 from \cite{forman1994hodge} tells us remarkably that these $E_j^k$ spaces are \emph{isomorphic} to the $e_j^k$ spaces of the filtration. The $E_j^k$ spaces are our real objects of interest, but the $e_j^k$ spaces are tractable to calculate. This is reminiscent of a standard methodology in algebraic topology where we prove difficult topological and analytic statements by turning them into algebraic statements. This will become our strategy to prove Lemma \ref{spec_seq_lemma}.

$\lambda^{-l}\rho^k_\lambda$ creates isomorphisms
\begin{align*}
Z_{j,l}^k \rightarrow \ &\widetilde{Z}_{j,l}^k \\
&:= \{|\psi_\lambda\rangle = |\psi_0\rangle + \lambda|\psi_1\rangle + \lambda^2|\psi_2\rangle + \dots \ : \ |\psi_i\rangle \in \mathcal{U}_{l+i}^k , \ d_\lambda|\psi_\lambda\rangle \in \lambda^j\mathcal{C}[\lambda]\} \\
Z_{j-1,l+1}^k \rightarrow \ &\lambda\widetilde{Z}_{j-1,l+1}^k \\
&:= \{|\psi_\lambda\rangle = \lambda|\psi_1\rangle + \lambda^2|\psi_2\rangle + \dots \ : \ |\psi_i\rangle \in \mathcal{U}_{l+i}^k , \ d_\lambda|\psi_\lambda\rangle \in \lambda^j\mathcal{C}[\lambda]\} \\
B_{j-1,l}^k \rightarrow \ &\widetilde{B}_{j-1,l}^k \\
&:= \lambda^{-j+1} d_\lambda \{|\psi_\lambda\rangle = |\psi_0\rangle + \lambda|\psi_1\rangle + \lambda^2|\psi_2\rangle + \dots \ : \ |\psi_i\rangle \in \mathcal{U}_{l-j+1+i}^{k-1} , \ d_\lambda|\psi_\lambda\rangle \in \lambda^{j-1}\mathcal{C}[\lambda]\} \\
&= \lambda^{-j+1} d_\lambda \widetilde{Z}_{j-1,l-j+1}^k
\end{align*}

Let $|\psi\rangle \in E_{j,l}^k$. Let
\begin{equation*}
|\psi_\lambda\rangle = |\psi\rangle + \lambda|\psi_1\rangle + \lambda^2|\psi_2\rangle + \dots
\end{equation*}
be the polynomial from the definition of $E_j^k$. Let $|\psi_{i,l}\rangle$ denote the projection of $|\psi_i\rangle$ onto $\mathcal{U}_l^k$, and write
\begin{align*}
|\psi_\lambda\rangle &= \bigg[|\psi\rangle + \sum_{i>0} \lambda^i|\psi_{i,l+i}\rangle\bigg] + \bigg[\sum_{i>0} \sum_{c\neq i} \lambda^i|\psi_{i,l+c}\rangle\bigg] \\
&= |\psi_\lambda^{(0)}\rangle + |\psi_\lambda^{(1)}\rangle
\end{align*}

\begin{proposition}\label{thm_7} \emph{(Theorem 7 from \cite{forman1994hodge})}

$|\psi_\lambda^{(0)}\rangle \in \widetilde{Z}_{j,l}^k$ and the map
\begin{align*}
\Gamma : E_{j,l}^k &\rightarrow \widetilde{Z}_{j,l}^k / (\widetilde{B}_{j-1,l}^k + \widetilde{Z}_{j-1,l+1}^k) \cong e_{j,l}^k \\
|\psi\rangle &\rightarrow [|\psi_\lambda^{(0)}\rangle]
\end{align*}
is an isomorphism.
\end{proposition}


\subsection{Example}

{\color{red} ROBBIE TO-DO: Filling in a 1D cycle.}


\subsection{Proof of Lemma \ref{spec_seq_lemma}}

We will apply the machinery of spectral sequences to the construction $\hat{\mathcal{G}}_m$ described in Section \ref{single_gadget_sec}. For this section, shorten the notation $\hat{\mathcal{G}}_m$ to $\hat{\mathcal{G}}$. Our real objects of interest for Lemma \ref{spec_seq_lemma} are the spaces $E_j^k$. Our plan is to compute the spaces $Z_{j,l}^k$, $B_{j,l}^k$, $e_{j,l}^k$ and use the isomorphism in Proposition \ref{thm_7} to analyze $E_j^k$. The isomorphism in Proposition \ref{thm_7} allows us to learn about the analytical spaces $E_j^k$ using easier algebraic techniques.

Recall that in Section \ref{single_gadget_sec}, we were concerned with the $(2m-1)$-homology, and we were filling in a $(2m-1)$-cycle by adding a gadget of $2m$-simplices. For the purposes of this section, let $k = 2m-1$. The relevant terms in the filtration are
\begin{align*}
\mathcal{C}^{k-1}(\hat{\mathcal{G}}) &= \mathcal{U}_0^{k-1} \supseteq\dots\supseteq \mathcal{U}_{k}^{k-1} \\
\mathcal{C}^{k}(\hat{\mathcal{G}}) &= \mathcal{U}_0^{k} \supseteq\dots\supseteq \mathcal{U}_{k+1}^{k} \\
\mathcal{C}^{k+1}(\hat{\mathcal{G}}) &= \mathcal{U}_0^{k+1} \supseteq\dots\supseteq \mathcal{U}_{k+2}^{k+1}
\end{align*}
with
\begin{align*}
\mathcal{U}_l^{k-1} &= \{0\} \ \forall \ l > k \\
\mathcal{U}_l^{k} &= \{0\} \ \forall \ l > k+1 \\
\mathcal{U}_l^{k+1} &= \{0\} \ \forall \ l > k+2
\end{align*}

Introduce the following notations:
\begin{itemize}
    \item $Z^k = \ker{d^k}$.
    \item $B^k = \im{d^{k-1}}$.
    \item Recall the definition of the gadget from Section \ref{single_gadget_sec}. Let $[\text{bulk}]$ denote the set of simplices which involve the central vertex $v_0$, and let $[\text{non-bulk}]$ be the complement of this set. It can be checked that $[\text{non-bulk}] \subseteq \hat{\mathcal{G}}$ is in fact a simplicial subcomplex, but $[\text{bulk}]$ is \emph{not}.
    \item Let $\Omega_j^k \subseteq \hat{\mathcal{G}}^k$ be the $k$-simplices of weights $\{1,\lambda,\dots,\lambda^{j-1}\}$. It can be checked that $\Omega_j \subseteq \hat{\mathcal{G}}$ is a simplicial subcomplex for each $j$, and $\mathcal{C}^k(\Omega_j) = (\mathcal{U}_{j+1}^k)^\perp$. Recalling Section \ref{single_gadget_sec}, $\Omega_0 \subseteq \hat{\mathcal{G}}$ is the original ``qubit complex'' before adding the gadget.
\end{itemize}

The following lemma, stated in generality, will prove useful.

\begin{lemma}\label{P_Q_lemma}
Let $\mathcal{P}$ be a simplicial complex and $\mathcal{Q} \subseteq \mathcal{P}$ a simplicial subcomplex. If $\mathcal{Q}$ has no $(k-1)$-cohomology, then
\begin{equation*}
\mathcal{C}^k(\mathcal{Q})^\perp \cap d^{k-1}(\mathcal{C}^{k-1}(\mathcal{Q})^\perp) = \mathcal{C}^k(\mathcal{Q})^\perp \cap B^k
\end{equation*}
\end{lemma}
\begin{proof}
It is clear that
\begin{equation*}
\mathcal{C}^k(\mathcal{Q})^\perp \cap d^{k-1}(\mathcal{C}^{k-1}(\mathcal{Q})^\perp) \subseteq \mathcal{C}^k(\mathcal{Q})^\perp \cap d^{k-1}(\mathcal{C}^{k-1}(\mathcal{P}))
\end{equation*}

Let $|\alpha\rangle \in \mathcal{C}^k(\mathcal{Q})^\perp \cap d^{k-1}(\mathcal{C}^{k-1}(\mathcal{P}))$. We must show that $|\alpha\rangle \in \mathcal{C}^k(\mathcal{Q})^\perp \cap d^{k-1}(\mathcal{C}^{k-1}(\mathcal{Q})^\perp)$. We know there is a $|\beta\rangle \in \mathcal{C}^{k-1}(\mathcal{P})$ with $|\alpha\rangle = d^{k-1}|\beta\rangle$. Now
\begin{equation*}
d^{k-1}(|\beta\rangle_{\mathcal{C}^{k-1}(\mathcal{Q})})_{\mathcal{C}^k(\mathcal{Q})} = 0
\end{equation*}
where the subscript denotes \emph{restriction}. Here comes the key step: $\mathcal{Q}$ has no $(k-1)$-cohomology, which implies that there exists a $|\gamma\rangle \in \mathcal{C}^{k-2}(\mathcal{Q})$ with
\begin{equation*}
|\beta\rangle_{\mathcal{C}^{k-1}(\mathcal{Q})} = (d^{k-2} |\gamma\rangle)_{\mathcal{C}^{k-1}(\mathcal{Q})}
\end{equation*}
Now $(d^{k-1} \circ d^{k-2}) |\gamma\rangle = 0$, so
\begin{equation*}
d^{k-1}(d^{k-2}|\gamma\rangle)_{\mathcal{C}^{k-1}(\mathcal{Q})} + d^{k-1}(d^{k-2}|\gamma\rangle)_{\mathcal{C}^{k-1}(\mathcal{Q})^\perp} = 0
\end{equation*}
Consider
\begin{equation*}
|\beta\rangle_{\mathcal{C}^{k-1}(\mathcal{Q})^\perp} - (d^{k-2} |\gamma\rangle)_{\mathcal{C}^{k-1}(\mathcal{Q})^\perp} \in \mathcal{C}^{k-1}(\mathcal{Q})^\perp
\end{equation*}
This has
\begin{equation*}
d^{k-1}\Big(|\beta\rangle_{\mathcal{C}^{k-1}(\mathcal{Q})^\perp} - (d^{k-2} |\gamma\rangle)_{\mathcal{C}^{k-1}(\mathcal{Q})^\perp}\Big) = |\alpha\rangle
\end{equation*}
\end{proof}

For the rest of the section, we will refer to the array with $l$ indexing the columns, increasing to the right, and $j$ the rows, increasing downwards.

\subsubsection{$Z_{j,l}^k$}

\begin{center}
\begin{tabular}{ c | c c c c c c }
$Z_{j,l}^k$ & $0$ & $\dots$ & $l$ & $\dots$ & $k+1$ & $l$ \\
\hline
$0$ & $\mathcal{U}_0^k$ & $\dots$ & $\mathcal{U}_l^k$ & $\dots$ & $\mathcal{U}_{k+1}^k$ & \\
$1$ & $\mathcal{U}_0^k$ & & $\mathcal{U}_l^k \cap (d^k)^{-1}(\mathcal{U}_{l+1}^{k+1})$ & & $\mathcal{C}^k([\text{bulk}])$ & \\
$2$ & $(d^k)^{-1}(\mathcal{U}_2^{k+1})$ & & $:$ & & $\mathcal{C}^k([\text{bulk}]) \cap Z^k$ & \\
$:$ & $:$ & & $:$ & & $\downarrow$ & \\
$:$ & $:$ & & $\mathcal{U}_l^k \cap (d^k)^{-1}(\mathcal{U}_{k+2}^{k+1})$ & & & \\
$:$ & $:$ & & $\mathcal{U}_l^k \cap Z^k$ & & & \\
$:$ & $:$ & & $\downarrow$ & & & \\
$k+2$ & $(d^k)^{-1}(\mathcal{U}_{k+2}^{k+1})$ & & & & & \\
$k+3$ & $Z^k$ & & & & & \\
& $\downarrow$ & & & & & \\
$j$ & & & & & &
\end{tabular}
\end{center}

$Z_{j,l}^k = \{0\} \ \forall \ l > k+1$ so we must only consider the columns $l = 0,\dots,k+1$. Recall $Z_{j,l}^k \supseteq Z_{j+1,l}^k \ \forall j$. That is, each entry of the $Z$-array \emph{contains} the entry immediately below. Moreover, $Z_{j,l}^k = Z_{n+3-l,l}^k \ \forall \ j > n+3-l$. That is, below the line $j+l=n+3$, the entries of each column do not change as we move down towards $j=\infty$. The first row $j=0$ is simply $Z_{0,l}^k = \mathcal{U}_l^k$. All ${k+1}$-chains involve at least one weight-$\lambda$ vertex, so $Z_{1,0}^k = \mathcal{U}_0^k$.

Let's look at the rightmost non-zero column $l=k+1$. The only relevant terms are $j=0,1,2$, below which the entry does not change with $j$. $Z_{1,k+1}^k$ are the $k$-chains supported on $k$-simplices of weight $\lambda^{k+1}$, and whose coboundaries are supported on $k+1$-simplices of weight $\lambda^{k+2}$. This is precisely the span of the $k$-simplices in $\mathcal{C}^k([\text{bulk}])$. (Note this is an abuse of notation since $[\text{bulk}]$ is \emph{not} a simplicial complex.) $Z_{2,k+1}^k$ are the $k$-cocycles supported on $k$-simplices of weight $\lambda^{k+1}$. This is $\mathcal{C}^k([\text{bulk}]) \cap Z^k$.

\subsubsection{$B_{j,l}^k$}

\begin{center}
\begin{tabular}{ c | c c c c c c }
$B_{j,l}^k$ & $0$ & $\dots$ & $l$ & $\dots$ & $k+1$ & $l$ \\
\hline
$0$ & $B^k$ & $\dots$ & $\mathcal{U}_l^k \cap B^k$ & $\dots$ & $\{0\}$ & \\
$1$ & $\downarrow$ & & $\downarrow$ & & $\mathcal{C}^k([\text{bulk}]) \cap B^k$ & \\
& & & & & $\downarrow$ & \\
$j$ & & & & & &
\end{tabular}
\end{center}

$B_{j,l}^k = \{0\} \ \forall \ l > k+1$ so we must only consider the columns $l = 0,\dots,k+1$. Recall $B_{j,l}^k \subseteq B_{j+1,l}^k \ \forall j$. That is, each entry of the $Z$-array \emph{is contained in} the entry immediately below. Claim \ref{final_l_B_clm} tells us about the final column $l=k+1$. $\mathcal{U}_{k+1}^{k-1}$ is zero, so in fact $B_{0,k+1}^k = \{0\}$. Claim \ref{mid_l_B_clm} tells us about the columns $l=0,\dots,k$. The first column $l=0$ is simply $B_{j,0}^k = B^k \ \forall j$.

\begin{claim}\label{final_l_B_clm}
$B_{j,k+1}^k = \mathcal{C}^k([\text{\emph{bulk}}]) \cap B^k \ \forall \ j \geq 1$
\end{claim}
\begin{proof}
This claim looks at the final colun $l = k+1$. All entries in this column are contained in $B_{j,k+1}^k \subseteq B_{\infty,k+1}^k \subseteq Z_{\infty,k+1}^k \subseteq Z_{1,k+1}^k = \mathcal{C}^k([\text{bulk}])$. Thus $B_{j,k+1}^k = \mathcal{C}^k([\text{bulk}]) \cap d^{k-1}(\mathcal{U}_{k+1-j}^{k-1})$, with $B_{\infty,k+1}^k = \mathcal{C}^k([\text{bulk}]) \cap B^k$.

Consider the $j=1$ entry $B_{1,k+1}^k = \mathcal{C}^k([\text{bulk}]) \cap d^{k-1}(\mathcal{U}_k^{k-1})$. Apply Lemma \ref{P_Q_lemma} with $\mathcal{P} = \hat{\mathcal{G}}$ and $\mathcal{Q} = [\text{non-bulk}]$. Note $\mathcal{C}^k([\text{non-bulk}])^\perp = \mathcal{C}^k([\text{bulk}])$. It can be checked that $[\text{non-bulk}]$ has no $(k-1)$-cohomology. {\color{red} Needs more explanation.} We get that $B_{1,k+1}^k = \mathcal{C}^k([\text{bulk}]) \cap B^k$. But $B_{0,k+1}^k \subseteq B_{j,k+1}^k \subseteq B_{\infty,k+1}^k \ \forall \ j \geq 1$ and $B_{\infty,k+1}^k = \mathcal{C}^k([\text{bulk}]) \cap B^k$, so $B_{j,l}^k = \mathcal{C}^k([\text{bulk}]) \cap B^k \ \forall \ j \geq 1$.
\end{proof}

\begin{claim}\label{mid_l_B_clm}
$B_{j,l}^k = \mathcal{U}_l^k \cap B^k \ \forall j \ \forall \ l=0,\dots,k$
\end{claim}
\begin{proof}
Fix the column $0 \leq l \leq k$. Consider the top entry in the column $B_{0,l}^k = \mathcal{U}_l^k \cap d^{k-1}(\mathcal{U}_l^{k-1})$. Apply Lemma \ref{P_Q_lemma} with $\mathcal{P} = \hat{\mathcal{G}}$ and $\mathcal{Q} = \Omega_{l-1}$. It can be checked that $\Omega_{l-1}$ has no $(k-1)$-cohomology. {\color{red} Needs more explanation.} (Note this is what fails for $l=k+1$.) We get that $B_{0,l}^k = \mathcal{U}_l^k \cap B^k$. But $B_{0,l}^k \subseteq B_{j,l}^k \subseteq B_{\infty,l}^k \ \forall j$ and $B_{\infty,l}^k = \mathcal{U}_l^k \cap B^k$, so $B_{j,l}^k = \mathcal{U}_l^k \cap B^k \ \forall j$.
\end{proof}

\subsubsection{$e_{j,l}^k$}

\begin{center}
\begin{tabular}{ c | c c c c c c }
$e_{j,l}^k$ & $0$ & $\dots$ & $l$ & $\dots$ & $k+1$ & $l$ \\
\hline
$0$ & $\mathcal{U}_0^k$ & $\dots$ & $\mathcal{U}_l^k$ & $\dots$ & $\mathcal{U}_{k+1}^k$ & \\
$1$ & $H^k(\Omega_1)$ & & $\{0\}$ & & $\mathcal{C}^k([\text{bulk}])$ & \\
$2$ & $H^k(\Omega_2)$ & & $\downarrow$ & & $\{0\}$ & \\
$:$ & $:$ & & & & $\downarrow$ & \\
$:$ & $:$ & & & & & \\
$k+2$ & $H^k([\text{non-bulk}])$ & & & & & \\
$k+3$ & $H^k(\hat{\mathcal{G}})$ & & & & & \\
& $\downarrow$ & & & & & \\
$j$ & & & & & &
\end{tabular}
\end{center}

$e_{j,l}^k = \{0\} \ \forall \ l > k+1$ so we must only consider the columns $l = 0,\dots,k+1$. The first row $j=0$ is simply $e_{0,l}^k = Z_{0,l}^k = \mathcal{U}_l^k$, and $e_{1,k+1}^k = \mathcal{C}^k([\text{bulk}])$; both of these follow straight from the definition. Claim \ref{final_l_e_clm} tells us that $e_{j,k+1}^k = \{0\} \ \forall \ j\geq 2$, and Claim \ref{mid_l_e_clm} tells us that all terms $l=1,\dots,k$, $j\geq 1$ are zero.

\begin{claim}\label{final_l_e_clm}
$e_{j,k+1}^k = \{0\} \ \forall \ j\geq 2$
\end{claim}
\begin{proof}
This claim looks at the final column $l = k+1$. For all $j\geq 2$,
\begin{align*}
e_{j,k+1}^k &= Z_{j,k+1}^k / B_{j-1,k+1}^k \qquad (Z_{j-1,k+2}^k = \{0\}) \\
&= \mathcal{C}^k([\text{bulk}]) \cap Z^k / \mathcal{C}^k([\text{bulk}]) \cap B^k
\end{align*}
To show $e_{j,l}^k = 0 \ \forall \ j\geq 2$, it is sufficient to show that $\mathcal{C}^k([\text{bulk}]) \cap Z^k \subseteq \mathcal{C}^k([\text{bulk}]) \cap B^k$. To this end, let $|\alpha\rangle \in \mathcal{C}^k([\text{bulk}]) \cap Z^k$.

Here comes the main idea in the proof. Recalling Section \ref{single_gadget_sec}, $\Omega_0 \subseteq \hat{\mathcal{G}}$ consists of $2^m$ copies of $S^k$ corresponding to the $m$-bit strings. For each copy of $S^k$ introduce an extra ``auxiliary'' vertex (of weight $1$) and connecting it with all vertices in this $S^k$, thus ``filling in the hole''. Denote the new objects after this operation with an overbar such as $\overline{\mathcal{G}}$. The effect of the auxiliary vertices is that $\overline{\mathcal{G}}$ has no $k$-cohomology.

$|\alpha\rangle \in \mathcal{C}^k([\text{bulk}])$ so $|\alpha\rangle_{\mathcal{C}^k(\Omega_0)} = 0$ and thus $|\alpha\rangle$, which we know is a cocycle in $\mathcal{G}$, is also a cocycle in $\overline{\mathcal{G}}$. But $\overline{\mathcal{G}}$ has no $k$-cohomology, so $|\alpha\rangle$ is in fact a \emph{coboundary} in $\overline{\mathcal{G}}$.

Now apply Lemma \ref{P_Q_lemma} with $\mathcal{P} = \overline{\mathcal{G}}$ and $\mathcal{Q} = \overline{[\text{non-bulk}]}$. We get that $|\alpha\rangle \in d^{k-1}(\mathcal{C}^{k-1}([\text{bulk}])) \subseteq B^k$.
\end{proof}

\begin{claim}\label{mid_l_e_clm}
$e_{j,l}^k = \{0\} \ \forall \ j\geq 1 \ \forall \ l=1,\dots,k$
\end{claim}
\begin{proof}
Fix the column $1\leq l\leq k$. Let's look at the row $j=1$. We aim to show $e_{1,l}^k = 0$.
\begin{align*}
e_{1,l}^k &= Z_{1,l}^k / (B_{0,l}^k + Z_{0,l+1}^k) \\
&= \mathcal{U}_l^k \cap (d^k)^{-1}(\mathcal{U}_{l+1}^{k+1}) / (\mathcal{U}_l^k \cap B^k + \mathcal{U}_{l+1}^k)
\end{align*}
To show $e_{1,l}^k = 0$, we must show that
\begin{equation*}
\mathcal{U}_l^k \cap (d^k)^{-1}(\mathcal{U}_{l+1}^{k+1}) \ \subseteq \ \mathcal{U}_l^k \cap B^k + \mathcal{U}_{l+1}^k
\end{equation*}
To this end, let $|\alpha\rangle \in \mathcal{U}_l^k \cap (d^k)^{-1}(\mathcal{U}_{l+1}^{k+1})$. We know that $d^k|\alpha\rangle \in \mathcal{U}_{l+1}^{k+1}$. Consider the subcomplex $\Omega_l$. $d^k|\alpha\rangle \in \mathcal{U}_{l+1}^{k+1}$ tells us that $(d^k|\alpha\rangle)_{\mathcal{C}^{k+1}(\Omega_l)} = 0$. That is, $|\alpha\rangle_{\mathcal{C}^k(\Omega_l)}$ is a \emph{cocycle} in $\Omega_l$.

We use the same main idea as in the proof of Claim \ref{final_l_e_clm}. Recalling Section \ref{single_gadget_sec}, $\Omega_0 \subseteq \hat{\mathcal{G}}$ consists of $2^m$ copies of $S^k$ corresponding to the $m$-bit strings. For each copy of $S^k$ introduce an extra ``auxiliary'' vertex (of weight $1$) and connecting it with all vertices in this $S^k$, thus ``filling in the hole''. Denote the new objects after this operation with an overbar such as $\overline{\mathcal{G}}$.

The effect of the auxiliary vertices is that $\overline{\mathcal{G}}$ has no $k$-cohomology. This includes $\overline{\Omega}_l$ for each $l$: these subcomplexes no longer have any $k$-cohomology.

$|\alpha\rangle \in \mathcal{U}_l^k$ and $l\geq 1$ so $|\alpha\rangle_{\mathcal{C}^k(\Omega_{l-1})} = 0$ and in particular $|\alpha\rangle_{\mathcal{C}^k(\Omega_0)} = 0$. We also know that $|\alpha\rangle_{\mathcal{C}^k(\Omega_l)}$ is a cocycle in $\Omega_l$. Thus $|\alpha\rangle_{\mathcal{C}^k(\overline{\Omega}_l)}$ is a cocycle in $\overline{\Omega}_l$. But $\overline{\Omega}_l$ has no $k$-cohomology, so $|\alpha\rangle_{\mathcal{C}^k(\overline{\Omega}_l)}$ is in fact a \emph{coboundary} in $\overline{\Omega}_l$.

Now apply Lemma \ref{P_Q_lemma} with $\mathcal{P} = \overline{\Omega}_l$ and $\mathcal{Q} = \overline{\Omega}_{l-1}$. We get that $|\alpha\rangle_{\mathcal{C}^k(\overline{\Omega}_l)} = (d^{k-1}|\beta\rangle)_{\mathcal{C}^k(\overline{\Omega}_l)}$ for some $|\beta\rangle \in \mathcal{C}^{k-1}(\overline{\Omega}_l) \cap \mathcal{C}^{k-1}(\overline{\Omega}_{l-1})^\perp$. But $\mathcal{C}^{k-1}(\overline{\Omega}_{l-1})^\perp = \mathcal{U}_l^{k-1}$ so $|\beta\rangle \in \mathcal{U}_l^{k-1}$ and in fact $|\alpha\rangle_{\mathcal{C}^k(\Omega_l)} = (d^{k-1}|\beta\rangle)_{\mathcal{C}^k(\Omega_l)}$. Thus $|\alpha\rangle = d^{k-1}|\beta\rangle + |\alpha'\rangle$ for some $|\beta\rangle \in \mathcal{U}_l^{k-1}$ and $|\alpha'\rangle \in \mathcal{U}_{l+1}^k$. This completes the proof that $e_{1,l}^k = 0$.

To argue about $e_{j,l}^k$ for $j>1$, we can (perhaps counterintuitively) invoke Proposition \ref{thm_7}. From the definition of $E_{j,l}^k$, it is clear that $E_{j,l}^k = 0 \implies E_{j',l}^k = 0 \ \forall \ j'\geq j$. Proposition \ref{thm_7} gives us an isomorphism $e_{j,l}^k \cong E_{j,l}^k$, thus $e_{1,l}^k = 0 \implies e_{j,l}^k = 0 \ \forall \ j\geq 1$. {\color{red} Can we see this more directly?}
\end{proof}

Let's interpret these proofs of Claims \ref{final_l_e_clm}, \ref{mid_l_e_clm} more closely. In Claim \ref{final_l_e_clm} we are given that $|\alpha\rangle$ is a cocycle, and we want to conclude that $|\alpha\rangle$ is in fact a coboundary. However, we cannot immediately do this since the complex has $k$-cohomology (and crucially so). The key step is to say that the cocycle $|\alpha\rangle$ has no support on the $k$-boundary of the complex, so \emph{it cannot tell} that there is $k$-cohomology. We are able to imagine closing all $k$-cycles with auxiliary vertices. Lemma \ref{P_Q_lemma} is then used to argue that this ``is not detected'' by $|\alpha\rangle$.

The interpretation of the proof of Claim \ref{mid_l_e_clm} is similar, albeit with an extra complication. In this case, we are given that $|\alpha\rangle$ is an \emph{approximate} cocycle, in the sense that $d^k|\alpha\rangle \in \mathcal{U}_{l+1}^{k+1}$. We want to conclude that $|\alpha\rangle$ is in fact an \emph{approximate} coboundary $|\alpha\rangle \in \mathcal{U}_{l+1}^k + \mathcal{U}_l^k \cap B^k$.

\bigskip
It remains to analyze the first column $e_{j,0}^k$. The definition gives $e_{j,0}^k = Z_{j,0}^k / (B_{j-1,0}^k + Z_{j-1,1}^k)$. But we know from Claim \ref{mid_l_e_clm} that
\begin{equation*}
Z_{j,l}^k = B_{j-1,l}^k + Z_{j-1,l+1}^k \ \forall \ j\geq 1 \ \forall \ l=1,\dots,k
\end{equation*}

First suppose $1\leq j\leq k+1$. Applying the above equality iteratively on the definition of $e_{j,0}^k$, we get
\begin{equation*}
e_{j,0}^k = \frac{Z_{j,0}^k}{B_{j-1,0}^k + B_{j-2,1}^k + \dots + B_{0,j-1}^k + Z_{0,j}^k}
\end{equation*}
This iteration works diagonally up and to the right on the table. But $B_{j-1,0}^k = B^k$ and $B_{j-1-l,l}^k = \mathcal{U}_l^k \cap B^k \ \forall \ 1\leq l\leq k$, so simply $B_{j-1,0}^k + B_{j-2,1}^k + \dots + B_{0,j-1}^k = B^k$. Further $Z_{j,0}^k = (d^k)^{-1}(\mathcal{U}_j^{k+1})$ and $Z_{0,j}^k = \mathcal{U}_j^k$, so for $1\leq j\leq k+1$
\begin{equation*}
e_{j,0}^k = \frac{(d^k)^{-1}(\mathcal{U}_j^{k+1})}{B^k + \mathcal{U}_j^k}
\end{equation*}

Applying the same logic for $e_{k+2,0}^k$ we get
\begin{equation*}
e_{k+2,0}^k = \frac{(d^k)^{-1}(\mathcal{U}_{k+2}^{k+1})}{B^k + \mathcal{C}^k([\text{bulk}])}
\end{equation*}

For $e_{k+3,0}^k$ we get
\begin{equation*}
e_{k+3,0}^k = \frac{Z^k}{B^k + \mathcal{C}^k([\text{bulk}]) \cap Z^k}
\end{equation*}
But Claim \ref{final_l_e_clm} tells us that $\mathcal{C}^k([\text{bulk}]) \cap Z^k = \mathcal{C}^k([\text{bulk}]) \cap B^k$ so simply $B^k + \mathcal{C}^k([\text{bulk}]) \cap Z^k = B^k$, and $e_{k+3,0}^k$ is the $k$-cohomology of the complex $\hat{\mathcal{G}}$ itself!
\begin{equation*}
e_{k+3,0}^k = Z^k/B^k = H^k(\hat{\mathcal{G}})
\end{equation*}

There is a similar interpretation for the spaces $\{e_{1,0}^k,\dots,e_{k+1,0}^k\}$ and $e_{k+2,0}^k$. For $1\leq j\leq k+1$, $e_{j,0}^k = (d^k)^{-1}(\mathcal{U}_j^{k+1}) / (B^k + \mathcal{U}_j^k)$. Quotienting by $\mathcal{U}_j^k$ is equivalent to restricting to $\mathcal{C}^k(\Omega_j)$. After we do this, $(d^k)^{-1}(\mathcal{U}_j^{k+1})$ becomes the $k$-cocycles in $\Omega_j$, denoted by $Z^k(\Omega_j)$, since $\mathcal{U}_j^{k+1} = \mathcal{C}^{k+1}(\Omega_j)^\perp$. $B^k$ naturally becomes the coboundaries in $\Omega_j$, denoted by $B^k(\Omega_j)$. Thus $e_{j,0}^k$ is precisely the \emph{$k$-cohomology} of $\Omega_j$.
\begin{equation*}
e_{j,0}^k = Z^k(\Omega_j) / B^k(\Omega_j) = H^k(\Omega_j)
\end{equation*}
By a similar logic, $e_{k+2,0}^k$ is precisely the $k$-cohomology of $[\text{non-bulk}]$.
\begin{equation*}
e_{k+2,0}^k = Z^k([\text{non-bulk}]) / B^k([\text{non-bulk}]) = H^k([\text{non-bulk}])
\end{equation*}
$\Omega_1,\dots,\Omega_{k+1}$ and $[\text{non-bulk}]$ in fact have isomorphic homologies, which are all in turn isomorphic to the homology $\mathcal{H}_m \cong (\mathbb{C}^2)^{\otimes m}$ of the qubit graph $\mathcal{G}_m$ before adding the gadget. (See Section \ref{single_gadget_sec}.) On the other hand, the full gadget $\hat{\mathcal{G}}_m$ has homology of dimension $2^m - 1$, since a single cycle $|\phi\rangle$ has been ``filled in''.

\subsubsection{$E_j^{2m-1}$}

At this point, let's revert back to the notation $2m-1=k$. From Proposition \ref{thm_7}, we can deduce the spaces $E_j^{2m-1}$. (Recall from Section \ref{single_gadget_sec} the definition of $\mathcal{H}_m \cong (\mathbb{C}^2)^{\otimes m}$.)
\begin{itemize}
    \item $E_0^{2m-1} \cong \mathcal{C}^{2m-1}(\hat{\mathcal{G}})$ (This is tautological.)
    \item $E_1^{2m-1} \cong H^{2m-1}(\Omega_1) \oplus \mathcal{C}^{2m-1}([\text{bulk}]) \cong \mathcal{H}_m \oplus \mathcal{C}^{2m-1}([\text{bulk}])$
    \item $E_j^{2m-1} \cong H^{2m-1}(\Omega_j) \cong \mathcal{H}_m \ \forall \ j= 2,\dots,2m$
    \item $E_{2m+1}^{2m-1} \cong H^k([\text{non-bulk}]) \cong \mathcal{H}_m$
    \item $E_j^{2m-1} \cong H^{2m-1}(\hat{\mathcal{G}}) \ \forall \ j\geq 2m+2$
\end{itemize}
In terms of eigenvalues, this means
\begin{itemize}
    \item There are many eigenvalues of order $\Theta(\lambda)$ corresponding to the span of the bulk simplices.
    \item There is a single eigenvalue of order $\Theta(\lambda^{2m+1})$ corresponding to the lifted state $|\phi\rangle \in (\mathbb{C}^2)^{\otimes m}$.
    \item There are $2^m-1$ eigenvalues equal to zero, corresponding to the harmonic states $|\psi\rangle \in (\mathbb{C}^2)^{\otimes m}$ orthogonal to $|\phi\rangle$.
\end{itemize}





